What Meaning-Form Correlation Has to Compose With

Compositionality is a widely discussed property of natural languages, although its exact definition has been elusive. We focus on the proposal that compositionality can be assessed by measuring meaning-form correlation. We analyze meaning-form correlation on three sets of languages: (i) artificial toy languages tailored to be compositional, (ii) a set of English dictionary definitions, and (iii) a set of English sentences drawn from literature. We find that linguistic phenomena such as synonymy and ungrounded stop-words weigh on MFC measurements, and that straightforward methods to mitigate their effects have widely varying results depending on the dataset they are applied to. Data and code are made publicly available.

==> tables/manual_annot.tex <==
\begin{tabular}{l l|r r|r r|r} %sdist tdist | rareeither rareboth syneither synboth preflen
\hline
\multicolumn{2}{c|}{\textbf{Distances}}&\multicolumn{2}{c|}{\textbf{Rare sense}}&\multicolumn{2}{c|}{\textbf{Synonym-based}}&\multirow{2}{*}{\textbf{Common start}}\\
\textbf{Meaning} & \textbf{Formal} & \textbf{Either} & \textbf{Both} & \textbf{Either} & \textbf{Both} \\ \hline
\multirow{2}{*}{$\cos$} & Lev.   & 42 & 0 & 100 & 100 & 0\\
                        & Lev. n & 34 & 1 & 88 & 88 & 10 \\
\multirow{2}{*}{$l_2$}  & Lev.   & 34 & 0 & 100 & 100 & 0 \\
                        & Lev. n & 32 & 0 & 98 & 98 & 0\\
\end{tabular}


==> tables/synthetic-languages-lm-old.tex <==
    \begin{tabular}{l l l l l}
    \hline
\textbf{Coeff.}          & \textbf{Estimate}    &  \textbf{Std. Error} & \textbf{t value}   & \textbf{Pr($>|t|$)}  \\ 
\hline
\textit{\small (Intercept)}     & 0.479757    &  0.002147   &  223.42   & $<$ 2e-16 \\
\hline
syn-2        & -0.149828   &  0.001384   &  -108.23  & $<$ 2e-16 \\
syn-3        & -0.207671   &  0.001384   &  -150.02   & $<$ 2e-16 \\
\hline
mwe-2        & 0.015240    &  0.001384   &  11.01    & $<$ 2e-16 \\
mwe-3        & 0.039637    &  0.001384   &  28.63    & $<$ 2e-16 \\
\hline
isp-1        & -0.052019   &  0.001598   &  -32.54   & $<$ 2e-16 \\
isp-2        & -0.078271   &  0.001598   &  -48.97   & $<$ 2e-16 \\
isp-3        & -0.096695   &  0.001598   &  -60.49   & $<$ 2e-16 \\
\hline
hol-2        & -0.007068   &  0.001648   &  -4.29    & 1.82e-05 \\
hol-3        & -0.028019   &  0.001648   &  -17.01   & $<$ 2e-16 \\
hol-4        & -0.060640   &  0.001648   &  -36.80   & $<$ 2e-16 \\
hol-5        & -0.203839   &  0.002794   &  -72.96   & $<$ 2e-16 \\
\hline
swap-1       & -0.074123   &  0.001648   &  -44.99   & $<$ 2e-16 \\
swap-2       & -0.063512   &  0.001648   &  -38.55   & $<$ 2e-16 \\
random-order & -0.076870   &  0.001648   &  -46.65   & $<$ 2e-16 \\

    \end{tabular}

==> tables/synthetic-languages-lm.tex <==
\begin{tabular}{lllll}
\hline
\textbf{Coeffs.}&\textbf{Estimate}&\textbf{Std. Error}&\textbf{t value}&\textbf{Pr($>|t|$)}\\\hline
\textit{\small(Intercept)} & 0.3571866 & 0.0002515 & 1420.187 & $<$2e-16\\
 syn-2 & -0.1271901 & 0.0001633 & -778.812 & $<$2e-16\\
 syn-3 & -0.1669668 & 0.0001736 & -961.582 & $<$2e-16\\ \hline
 mwe-2 & 0.0093713 & 0.0001726 & 54.307 & $<$2e-16\\
 mwe-3 & 0.0247616 & 0.0001707 & 145.079 & $<$2e-16\\ \hline
 isp-1 & -0.0324466 & 0.0001899 & -170.901 & $<$2e-16\\
 isp-2 & -0.0509883 & 0.0001936 & -263.385 & $<$2e-16\\
 isp-3 & -0.0635285 & 0.0001968 & -322.727 & $<$2e-16\\ \hline
 hol-2 & -0.0057629 & 0.0001893 & -30.448 & $<$2e-16\\
 hol-3 & -0.0291452 & 0.0001918 & -151.946 & $<$2e-16\\
 hol-4 & -0.0726029 & 0.0002014 & -360.523 & $<$2e-16\\
 hol-5 & -0.2734605 & 0.0022557 & -121.232 & $<$2e-16\\ \hline
 strict-order & 0.0002108 & 0.0001956 & 1.077 & 0.281\\
 swap-1 & 0.0001893 & 0.0001957 & 0.967 & 0.333\\
 swap-2 & 0.0002143 & 0.0001957 & 1.095 & 0.274\\ \hline
\end{tabular}

==> tables/table-defs-all.tex <==
\npdecimalsign{.}

\nprounddigits{5}

\begin{tabular}{ l  l l | n{2}{5} n{2}{5} n{2}{5} n{2}{5}}
    \multicolumn{3}{c|}{\textbf{Distances}} & \multicolumn{4}{c}{\textbf{Control Operations}} \\
    \textbf{Embeddings} & \textbf{Meaning} & \textbf{Form} & \textbf{None} & \textbf{Stop-words} & \textbf{Synonyms} & \textbf{Paraphrases} \\ \hline \hline
    \multirow{8}{*}{\textbf{word2vec}} & \multirow{4}{*}{$\cos$} & Lev. & 0.016906309115858928 &  0.009326709420716091 &  0.016953 & 0.026041\\
                                       &                         & Lev. n & 0.014297867010866282 & 0.013724686555119844 & 0.016156 & 0.006381 \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\
                                       & \multirow{4}{*}{$l_2$}  & Lev. & \\
                                       &                         & Lev. n & \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\ \hline
    \multirow{8}{*}{\textbf{fastText}} & \multirow{4}{*}{$\cos$} & Lev. & 0.03110060198704507 & 0.02753648640100917 & 0.031070 & 0.044123\\
                                       &                         & Lev. n & 0.016089142174786162 &  0.02238587400533237 & 0.012583 &  \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\
                                       & \multirow{4}{*}{$l_2$}  & Lev. & \\
                                       &                         & Lev. n & \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\ \hline
    \multirow{8}{*}{\textbf{\textsc{g}lo\textsc{v}e 840\textsc{b}}} & \multirow{4}{*}{$\cos$} & Lev. &  0.046696391099520174 & 0.05121040391558046 & 0.047099 & 0.057019\\
                                       &                         & Lev. n & & 0.020981382299674584 & & -0.019701 \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\
                                       & \multirow{4}{*}{$l_2$}  & Lev. & \\
                                       &                         & Lev. n & \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\ \hline
    \multirow{8}{*}{\textbf{\textsc{g}lo\textsc{v}e 6\textsc{b}}} & \multirow{4}{*}{$\cos$} & Lev. &  0.021265281323303752 &  0.027600495179112627 & 0.021333 & 0.031095 \\
                                       &                         & Lev. n & & 0.013432678641566349 & & -0.011062 \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\
                                       & \multirow{4}{*}{$l_2$}  & Lev. & \\
                                       &                         & Lev. n & \\
                                       &                         & \textsc{ted} & \\
                                       &                         & \textsc{ted} n & \\ \hline
     
\end{tabular}
